Informing clinical assessment by contextualizing post-hoc explanations of risk prediction models in type-2 diabetes

Medical experts may use Artificial Intelligence (AI) systems with greater trust if these are supported by contextual explanations that let the practitioner connect system inferences to their context of use. However, their importance in improving model usage and understanding has not been extensively studied. Hence, we consider a comorbidity risk prediction scenario and focus on contexts regarding the patients clinical state, AI predictions about their risk of complications, and algorithmic explanations supporting the predictions. We explore how relevant information for such dimensions can be extracted from Medical guidelines to answer typical questions from clinical practitioners. We identify this as a question answering (QA) task and employ several state-of-the-art LLMs to present contexts around risk prediction model inferences and evaluate their acceptability. Finally, we study the benefits of contextual explanations by building an end-to-end AI pipeline including data cohorting, AI risk modeling, post-hoc model explanations, and prototyped a visual dashboard to present the combined insights from different context dimensions and data sources, while predicting and identifying the drivers of risk of Chronic Kidney Disease - a common type-2 diabetes comorbidity. All of these steps were performed in engagement with medical experts, including a final evaluation of the dashboard results by an expert medical panel. We show that LLMs, in particular BERT and SciBERT, can be readily deployed to extract some relevant explanations to support clinical usage. To understand the value-add of the contextual explanations, the expert panel evaluated these regarding actionable insights in the relevant clinical setting. Overall, our paper is one of the first end-to-end analyses identifying the feasibility and benefits of contextual explanations in a real-world clinical use case.

==> submissions/AIM_original/tex/abstract.tex <==

% \todotip[sc] { this says it is to be edited by shruthi - has that been done?  the email says the abstract is ready.}
% %SC yes I addressed above and edited to make the claims clearer 
%SC Move to resuls, contextualization overlaps and themes overlap 
%SC Guideline QA - coverage of guidelines + what is accuracy of guideline QA 
Medical experts can use Artificial Intelligence (AI) systems with greater trust if model inferences about patients are connected to explanations, including the context of use. We consider the problem of risk prediction, an issue of diagnostic and interventional importance to clinicians, to analyze the tools and processes required to make AI models more useful. 
To satisfy the needs of clinicians, through a continuous engagement with medical experts we developed a \textit{contextual explanation} approach that focuses on combining insights from different domain knowledge sources to make AI predictions more useful.
In particular, we studied the feasibility and benefits of providing such additional explanations around AI model predictions and standard post-hoc explanations to clinicians by extracting and supporting knowledge from authoritative literature such as medical guidelines.
As a case study, we built black-box AI models and post-explainers to predict and identify the drivers of risk of chronic kidney disease ({\ckd}) - a common type-2 diabetes {\dm} comorbidity. 
Crucially, we developed a novel unsupervised and knowledge-augmented question answering (QA) method to present contexts around these predictions by supporting answers to types of clinically relevant questions. 
Based on expert feedback, the context enhancements focus on the dimensions of \textit{the patients' clinical state, AI predictions about their risk of complications, and algorithmic explanations supporting the predictions}. 
We currently use these contexts to answer $175$ questions of $5$ different types on $20$ prototypical patients.
Furthermore, with the aid of a prototype dashboard presenting such contexts, we conducted structured feedback sessions with $4$ experts to identify their needs and performed thematic analysis. We evaluate our methods by both qualitative and quantitative analysis. From our structured feedback sessions, we found $4$ themes covering $11$ sub-themes of interest to make risk predictions more useful that also indicate the importance of \textit{contextual explanations}. The guideline question-answering approach results demonstrate the value of knowledge and rule augmentations in enhancing language models' capabilities. The identified gaps from these results also provide a pathway for subsequent research in this domain.
Overall, our paper is one of the first end-to-end reports on applying various principles of user-driven explainability to a real world clinical use case and the practical considerations at bridging the gap between AI models and their usage by clinicians. Our approach to contextual explanations is interdisciplinary, combines insights from experts and domain knowledge, and %supported by qualitative and quantitative analysis
aims to lay the foundation for future research to make AI models more useful to clinicians.


\iffalse
Medical experts can use Artificial Intelligence (AI) systems with greater trust if model inferences about patients are connected to explanations including the context of use. We consider the problem of risk prediction, an issue of diagnostic and interventional importance to clinicians, to analyze the tools and processes required to make AI models more useful. In particular,  we constructed black-box AI models to predict the risk of chronic kidney disease ({\ckd}) - a common type-2 diabetes {\dm} comorbidity and augmented these predictions by post-hoc model explanations of the factors contributing to the risk. We then developed a novel knowledge augmented question answering method to present contexts around these predictions, by supporting answers to types of clinically relevant questions. The context enhancements focus on the   dimensions of \textit{the patients' clinical state, AI predictions about their risk of complications, and algorithmic explanations supporting the predictions}. We used a prototype dashboard to conduct structured feedback sessions with $4$ experts, wherein we found $4$ themes covering $11$ sub-themes of interest to make risk predictions more useful.
We currently use these contexts to answer $150$ questions of $5$ different types on $20$ prototypical patients. In summary, our results identify the needs of clinicians in risk prediction settings and then explore how such requirements can be satisfied by augmenting knowledge from authoritative literature such as guidelines. To address these needs, we develop a \textit{contextual explanation} approach, that focuses on combining insights from different domain knowledge sources to make predictions more useful.
\fi


\begin{comment}
Adoption of automated systems in high-precision domains like healthcare is enhanced when explanation features are included. Past studies, and our ongoing interactions with practitioners, suggest that medical experts can use Artificial Intelligence (AI) systems with greater trust if model inferences about patients are connected to explanations tied to the context of use and accepted domain knowledge. In this paper, we consider the problem of risk prediction, an issue of diagnostic and interventional importance to clinicians, to analyze the tools and processes required to make AI models more useful. We conducted interviews with a clinical expert on our team to understand clinicians' workflow, especially concerning the usage of risk prediction modules, and identified various scenarios of interest. Our interviews indicated that clinicians consult different knowledge sources while using such data-driven scores to make decisions. To address these needs, we propose a new term in this paper, \textit{contextual explanations}, that focus on combining insights from different domain knowledge sources to make predictions more useful. As a setting, we have designed methods to provide context from different domain knowledge sources in a type-2 diabetes ({\dm}) use case, where we constructed black-box AI models to predict the risk of chronic kidney disease ({\ckd}) - a common {\dm} comorbidity. These AI models were further backed by post-hoc model explanations that explained the factors contributing to the risk. To make the risk predictions and their associated feature importances more useful and explainable, we have designed a multi-method approach to present context around these predictions along the dimensions of \textit{the patients' clinical state, AI predictions about their risk of complications, and algorithmic explanations supporting the predictions}, as answers to a list of clinically relevant questions. Our multi-method approach comprises information retrieval, templated question and answer generation, and question-answering (QA) modules that can extract relevant contexts from different domain knowledge sources, including patient data, medical ontologies, and clinical guidelines. As part of this approach, we have also developed a novel, knowledge-modulated, deep-learning question-answering system to extract relevant knowledge from clinical guidelines. We report accuracy values for the risk prediction and post-hoc explanation models, and conducted qualitative coverage analysis and quantitative accuracy analysis on the outputs of the QA module to understand the importance of extracted information from guidelines. Finally, we have created a prototype dashboard to present the predictions of the risk models along the contextual explanations around the three identified dimensions of interest. We used the dashboard as an aid to conduct structured feedback sessions with $4$ experts to determine their needs while using such context and explanation-enabled AI models in practice. We uncovered $4$ themes covering $11$ sub-themes of interest for the clinicians, where further contextual information about the patients, diagnosis, and prognosis would make risk prediction models and their explanations more applicable. We also analyzed the ability of the guidelines to support these themes and find that guidelines can act as a valuable source of information that can be realistically extracted on-demand to augment other patient information and support the needs of the clinicians while using risk prediction models in practice. We currently use these contexts to answer $150$ questions of $5$ different types, for a total of $20$ prototypical patients. In summary, our results identify the needs of clinicians in risk prediction settings and then explore how such requirements can be satisfied by augmenting knowledge from authoritative literature such as guidelines.
\end{comment}
%SC reminder to correct the question number based on evaluations 

%Stacking unused info
% While some of this information could be extracted from cohort analysis and/or patient summarization, additional answers could be provided from published medical knowledge. Clinical guidelines are one of the most trusted sources of such knowledge, as supported by their position in the scientific knowledge pyramid. 
%  In this paper, we analyzed the usefulness of such guidelines to provide the required contextual explanations around risk predictions.
%SC removing the SHAP values detail
%using Shapley values.


% SC I think this has already been said
% Finally, our multi-method approach to providing context around entities of interest in the risk prediction setting, the patient, their predicted risk, and explanations of their risk, was vetted and improved by multiple rounds of clinical interviews.


% wherein they consult different sources to make decisions. To enable adoption of  ever-improving AI risk prediction models in practice, we are exploring techniques to contextualize such models along three dimensions of interest: \textit{the patients' clinical state, AI predictions about their risk of complications, and algorithmic explanations supporting the predictions}. 

% We design a multi-method approach to present context around these dimensions and do so in type-2 diabetes ({\dm}) use case, where we predict the risk of chronic kidney disease ({\ckd}) - a common {\dm} comorbidity.  Within our approach, we include risk prediction models for CKD, post-hoc explainers that provide interpretations for the predictions, and other natural-language, question-answering modules which operationalize domain knowledge from clinical practice guidelines, patient data, and medical ontologies to provide context. The risk predictions, explanations, and additional context are then presented on a user-friendly risk prediction dashboard. 

% Using the risk-prediction dashboard as an aid, we conducted expert panel interviews with clinicians, walking them through our use case and the contexts we support, to understand the effectiveness of our approach in enabling better clinical decision-making in risk prediction settings. We report results of the thematic analysis from these sessions. On a high level, we found that clinicians were looking for \textit{additional clinical context to interpret the patient's risk prediction score and the factors that affect the score}. Some of these contexts were covered well by the type-2 diabetes guidelines, like coverage of recent antidiabetic drugs and their comorbid risks, updated treatment and management suggestions, and references for factors that influence or correlate with {\ckd} risk. We found that the other contexts were solved by a better connections to patient data. In addition, to the thematic analysis, we also report accuracy scores for each of the sub-modules of our multi-method approach. Overall, our ongoing approach covers multiple knowledge sources, blends knowledge to explain data and predictions to PCPs, and is a step towards better user-centered explainability for high-risk clinical settings.



==> submissions/AIM_original/tex/clinical_scenario.tex <==
%  \todotip[PC]{lead}
Risk prediction models can be consumed by a broad spectrum of clinicians with differing roles and experience, e.g. a specialist vs a primary-care physician. Depending on their roles, the needs, and thereby the desired functionality from a risk prediction contextualization standpoint, can be different. As such, we conducted expert interview sessions
to understand the clinical use-case and determine the context of AI tools. More specifically,  we followed a sequence of %standard 
user-centric research principles~\cite{liao2020questioning}, to
(1) define the scope of our tool's capabilities, (2) identify the end-user/target persona who would most benefit from our tool, and (3) scope the most relevant %and realistic
contexts and usage scenarios for our tool.

Through our interviews, we identified primary-care physcians, especially those with lesser years of experience, to be the persona who may most benefit from such contextualizations. We also walkthrough typical contexts of {\dm} patient care by clinician type and patient characteristics,  and understand how risk predictions %and better forecasting 
can help clinicians improve patient care planning. 
Interestingly, while current literature~\cite{wang2019designing} on designing healthcare models points to a user-centered approach, from this understanding of clinician workflows, we identified the importance of grounding such work in clinical scenarios (see Fig~\ref{fig:dashboard}). 
We found that dashboards containing contextual explanations around risk prediction, presented as a drill-down analysis of the patient EHR records, can be used by clinicians in different manners. These manners depend on whether the patient is seeing the clinician for the first time and/or for the first diagnosis (where they are more interested in creating their mental model of the patient's diagnosis and understanding the causes for their risk), or if the patient is returning to the clinician with a previously established diagnosis (where clinicians may be more interested in understanding the temporal elevation of risk over time and planning appropriate interventions). 
Based on these understandings, we formalize our use case to \textit{provide contextual explanations to a PCP around the predicted risk of {\ckd} among new {\dm} patients at their first diagnosis}.
In the following sections, we describe the constructed risk models and structured, scenario-based interviews with an expert panel to uncover the contextual dimensions that will enable them to use the AI models in practice.


\begin{figure*}[!htbp]
\centering
\includegraphics[trim=0 0 0 30,width=\linewidth]{images/PCP-workflow-diagram-condensed.png}
\caption{Illustration of findings for a Primary Care Physician (PCP) - one target persona among clinicians - whose workflow is dependent on the patient context and the clinician-patient history. We show an example scenario where the predicted risk for a returning patient has increased since the last visit. This context and the PCP's mental model drive the PCP's following actions, such as differential treatment decisions made by probing reasons for the increased risk.}

\label{fig:dashboard}
\end{figure*}


==> submissions/AIM_original/tex/discussion_remaining.tex <==
%discussion - but rough start so not to render on UI

Additionally from the expert panel sessions we see that a combination of content from domain knowledge sources,  patient context and model details are necessary to improve clinicians trust and uptake of risk prediction tools. Further while some requests from the clinicians might be easily addressable by content presentation, others require feature development either improving existing modules we currently support or building new ones. Thus, the high level themes and sub themes from expert panel studies can be considered to be indicative of features that would improve usability and uptake of risk prediction tools in general and as general directions for us to implement. 
Enhance real-world usability and there is value in including user feedback at every stage of the development cycle ( cite park ET al) 

Cite the Ui presentation paper for which sections were most important and link them to the themes 

==> submissions/AIM_original/tex/results_risk.tex <==
% \todotip[PC]{Lead}
We present the performance of the risk prediction models in Tab. ~\ref{tab:resultsCKD}. As the table shows, while GRU performs the best overall, depending on the use case, we may want to prefer other models. For the purposes of this paper, we chose MLP as our risk prediction model to benefit from the higher recall (such that the probability of false negatives is low) and high brier-score (to allow a more natural interpretation of our model outputs for clinicians), while still achieving an acceptable level of overall performance (AUC-ROC = $0.59$).


\begin{table}[ht!]
  \caption{Results of CKD risk from different prediction models}
  \centering
  %\todotip[PC]{add CI}
  \label{tab:resultsCKD}
  \begin{tabular}{lccccc}
    \toprule
    Method & Precision & Recall & AUC-ROC & AUC-PRC & Brier\\
    \midrule
    %One-class SVM & & \\
    LR    &  0.333 & 0.023  & 0.582 & 0.215 &  0.127 \\
    MLP   &  0.139 &  {\bf 0.977} & 0.587 & 0.224 & {\bf 0.621}  \\
    LSTM  &  {\bf 0.242} &  0.442 & {\bf 0.678} & 0.263 & 0.208  \\
    GRU   &  0.240  &  {\bf 0.605} & 0.677 & {\bf 0.311} & 0.220   \\
  \bottomrule
\end{tabular}
\end{table}

\begin{figure*}[!htbp]
    \centering
    % \begin{subfigure}{0.74\textwidth}
    %   \includegraphics[width=\linewidth]{./images/shap_bar_proto_CKD_w360_v1.png}
    % \caption{Feature importance}
    % \label{fig:shap:bar_proto}    
    % \end{subfigure}
    % \hspace{-1.5em}
    % \begin{subfigure}{0.257\textwidth}
    %  \adjincludegraphics[width=\linewidth,trim={{.65\width} 0 0  0},clip]{./images/shap_summary_proto_CKD_w360_v1.png}
    %   %\includegraphics[trim=10cm 0 0 0,clip=true,totalwidth=0.9\linewidth]{./images/shap_summary_proto_{\ckd}_w360_v1.png}
    %     \caption{Feature Impact}
    %     \label{fig:shap:violin_proto}
    % \end{subfigure}
    \includegraphics[width=\linewidth]{./images/feature_summary.pdf}
    \vspace{-2em}
        \caption{Feature importance for {\ckd} prediction among {\numproto} prototypical patients using SHAP (left), showing absolute importance, and (right) showing feature impact on model prediction w.r.t. presence/absence of features}
        \label{fig:shap:summary_proto}
\end{figure*}

Feature importance for risk factors found by algorithmic explainers can be further contextualized, as mentioned previously.
The left hand column of Fig.~\ref{fig:shap:summary_proto} shows the top $20$ features for the set of {\numproto} prototypical patients under investigation. These prototypical patients are all found to be at high-risk for {\ckd} and hence, would be interesting to clinicians within the scope of this {\dm} and {\ckd} use case. %(\textbf{Q. 1}). 
For these prototypical patients, we present aggregated feature importances, as seen in Tab. \ref{tab:protosummary_appendix}, to account for HIPAA restrictions.  We can see that demographic features, such as age and the presence of other disorders, such as `other skin disorders,' were found to be important for the {\ckd} risk prediction. 
The right side of Fig. ~\ref{fig:shap:summary_proto} shows an alternate view of the same, providing a view into the spread of individual importances. From this deeper view, we can see that features such as `calculus of urinary tract' could be the most important drivers of risk for some patients. Such results further support our need to personalize features found to be important for the risk predictions. 
% contextualization

While insights about the importance of such features are helpful, such clinical and patho-physiological features may need further contextualization for clinicians. Our structured feedback sessions found that clinicians found the contextual explanations we support around these features helpful, and we cover some of this next. 

\begin{table}
\caption{Entire baseline description summary (generated using Tableone library~\cite{pollard2018tableone}) of the 20 prototypical patients highlighting the demographic and diagnoses counts. We report the disease diagnoses by their higher-level disease groupings (e.g. for {\dm} the higher-level code is endocrine, nutritional and metabolic disorders). We highlight the conditions that are most prevalent amongst the patients ($> 50\%$).}
% -- CASE WHEN age_at_onset>=19 AND age_at_onset<=44 THEN 1 ELSE 0 END AS AGE_GRP_Y,
% -- CASE WHEN age_at_onset>=45 AND age_at_onset<=54 THEN 1 ELSE 0 END AS AGE_GRP_M,
% -- CASE WHEN age_at_onset>=55 AND age_at_onset<=64 THEN 1 ELSE 0 END AS AGE_GRP_O
\centering
\label{tab:protosummary_appendix}
 \begin{tabular}{lcc}
\toprule
                                                                       Feature                  &     Overall \\
\midrule
n &          20 \\
Age at onset 45-54, n (\%) &    4 (20.0) \\
\textbf{Age at onset $\geq$ 55, n (\%)} &   \textbf{15 (75.0)} \\
Age at onset $\leq$ 44, n (\%) &     1 (5.0) \\
SEX - FEMALE, n (\%) &    7 (35.0) \\
Mood disorders, n (\%)  &    3 (15.0) \\
Diseases of the blood and blood-forming organs, n (\%)  &    3 (15.0) \\
\textbf{Diseases of the circulatory system, n (\%)} &   \textbf{17 (85.0)} \\
Diseases of the digestive system, n (\%) &    6 (30.0) \\
Diseases of the genitourinary system, n (\%) &    9 (45.0) \\
\begin{tabular}[c]{@{}l@{}} \textbf{Diseases of the musculoskeletal system} \\ \textbf{and connective tissue, n (\%)} \end{tabular}  &   \textbf{12 (60.0)} \\
Diseases of the nervous system and sense organs, n (\%)  &    9 (45.0) \\
\textbf{Diseases of the respiratory system, n (\%)} &   \textbf{11 (55.0)} \\
Diseases of the skin and subcutaneous tissue, n (\%) &    7 (35.0) \\
\begin{tabular}[c]{@{}l@{}} \textbf{Endocrine; nutritional; and metabolic} \\ \textbf{ diseases and immunity disorders, n (\%)} \end{tabular} &  \textbf{20 (100.0)} \\
Infectious and parasitic diseases, n (\%) &   10 (50.0) \\
Injury and poisoning, n (\%) &    4 (20.0) \\
Mental Illness, n (\%)  &    3 (15.0) \\
Neoplasms, n (\%)  &    6 (30.0) \\
\begin{tabular}[c]{@{}l@{}} Symptoms; signs; and ill-defined conditions \\ and factors influencing health status, n (\%) \end{tabular} &   10 (50.0) \\
\bottomrule
\end{tabular}
\end{table}




==> submissions/AIM_original/tex/risk_method.tex <==
\subsection{Risk Prediction Models}
\label{ssub:risk_model}
% \todotip[PC]{lead}
From the constructed cohort and the aforementioned use-case scenario for a target definition (Sec. \ref{sec:use-case}), we built a ML model for predicting risk, based on the highest predictive accuracy and other appropriate metrics for the use case, such as favoring models with a higher recall. 
% relevance to the context. %To this end, w
We used DPM 360~\cite{dpm360}, an open-source, reusable, disease progression model training package, to train and compare a suite of classification models on the patients' demographic and diagnosis history to predict future complications.
In this paper, we only used the demographic and diagnostic features to model risk. Furthermore, to handle the temporal features, for some of our models, such as Logistic Regression (LR) and Multi-layer perceptron (MLP), we used temporally aggregated features (summation). 
We also compared two state-of-the art Recurrent Neural Networks (RNN) where temporal history can be handled in a more natural manner, viz., Long-Short Term Memory (LSTM) and Gated Recurrent Units (GRU). All model implementations are available via DPM360 including classical ML models (backed by scikit-learn) and deep learning models (custom built for DPM).
In this paper, 
we split the data according to a train-validation-test split (70-10-20). Using the best performing models on the validation set, we present our results on the hold-out test set.
 Since the data is imbalanced, we selected the models based on the best AUC-ROC and AUC-PRC from the validation set. We also evaluate the models based on precision, recall, and brier score~\cite{rufibach2010use}. Deep learning networks are known to be under-calibrated and the last metric measures how well the model is calibrated, i.e., it measures the probabilistic interpretation of risk prediction. In other words, if a model predicts a $0.7$ risk for a patient, brier score measures how well that translates to a $70\%$ chance of the patient developing the complication.
The hyper-parameters for the deep-learning models were selected using a grid search strategy varying batch sizes  $\lbrace 8, 16, 32, 128 \rbrace$, number of layers $\lbrace 1, 2, 3 \rbrace$, and dropout $\lbrace 0.0, 0.1, 0.2 \rbrace$ along with standard initialization and using ADAM as the optimizer of choice. 
% \todotip[PC]{add the hyper-parameter sweep}


% The models include both classical such as Logistic Regression (LR) as well as modern deep learning methods  such as Multi-Layer Perceptron (MLP), Long-Short Term Memory (LSTM), and Gated Recurrent Units (GRU). We followed standard ML methods for model evaluation and, based on our results, we selected MLP as our model choice to balance recall with overall performance. For further details, see Appendix~\ref{ssub:risk_model}

\subsection{Post-hoc Explainer Models}
% \todotip[PC]{lead}

While some of the classical algorithms considered in Section~\ref{ssub:risk_model} are inherently interpretable with easy access to the features deemed important for the model (such as LR), several of the deep learning models are black-box models. 
To extract feature importances from such models, we used post-hoc explainers which have been found to be favored by clinicians in past studies~\cite{tonekaboni2019clinicians}.
In particular, we used the well accepted SHAP algorithm~\cite{lundberg2018explainable} to find feature importance. The algorithm uses game-theoretic principles to identify importance of features by ascertaining the dip in performance of the model with and without access to the feature at the personalized level. 
Such personalized feature importance is key so that our overall risk prediction presentations are more actionable for the clinicians by allowing them to focus on the particular attributes of the patients that are driving their risk.

Typically, clinician time is costly and hard to obtain. Thus to let clinicians focus on some of the most `interesting' patients, we apply Protodash, a post-hoc sample selection method~\cite{gurumoorthy2019efficient}, to select a set of prototypical or representative patients from the high risk category. Prototypical patients from Protodash naturally spans the varied set of patient characteristics for the selected sub-group. This also allows the clinician to build trust in using the AI models by inspecting the different patient modalities of the dataset without having to inspect the entire dataset.


==> submissions/AIM_original/tex/use_case.tex <==
% \todotip[PC]{lead}
% \explannote[PC]{done}

Diabetes is one of the top five chronic diseases affecting the adult population in the US~\cite{cdcT2D}. 
Diabetes management involves monitoring for and treating %the 
related comorbid conditions. 
Effective and timely prediction of such conditions can lead to an overall improvement in the quality of care. We focus on {\dm} and use machine learning (ML) models to predict the risk of developing certain {\dm} comorbid complications. Among these, {\ckd}, a commonly occurring micro-vascular complication of {\dm}, is one of the leading causes of death in the US~\cite{cdcCKD}, with an estimated $37$ million cases in the US (who are mostly undiagnosed) and cost medicare in 2018 $81.1B$, and end stage renal disease an additional $36.6B$. Typically, actions to prevent onset of {\ckd} among {\dm} patients revolve around proper disease control,  including close disease monitoring, proper treatment adherence, and patient education. Incorporating accurate risk prediction of {\ckd} in the clinical workflow can lead to more timely actions, potentially delaying the onset of {\ckd}, and in some cases, preventing its progression.
While such predictions could be of use along various time-points of the patients' {\dm} prognosis, in this paper, we predict the risk of developing {\ckd} within 360 days of {\dm} onset. 
Under this use case, we explore strategies to provide context around interventions for particular patients, and explain their {\dm} state and individual risk factors.
We conduct our analysis on claims sub-component of the Limited IBM MarketScan Explorys Claims-EMR Data Set (LCED), covering both administrative claims and EHR data of over $5$ million commercially insured patients between 2013 and 2017.
Medical diagnoses are encoded %in the database 
using International Classification of Diseases (ICD) codes. 
We selected only those {\dm} patients (with ICD9 codes 250.*0, 250.*2, 362.0, and ICD10 code E11)  that satisfied the following criteria as our cohort.
 Only {\dm} patients with the following criteria are included:% in the study:
\begin{itemize}
  \item have had two or more visits with {\dm} diagnosis,
  \item  were enrolled continuously for $12$ months prior to %initial 
{\dm} diagnosis,% with {\dm}. 
  \item  number of visits for {\dm}  is greater than those for other forms of diabetes such as \texttt{T1D}, and
  \item  age at the initial {\dm} diagnosis is between 19-64 years.
\end{itemize}

Among {\dm} patients, we use the first diagnosis of chronic kidney disease ({\ckd}) (ICD10 N18 or ICD9 585.*, 403.*) after the initial diagnosis of {\dm} as the outcome to predict. %In this paper, a
At the time of the first {\dm} diagnosis, we predict the risk of the patient developing {\ckd} within $1$ year using Clinical Classifications Software (CCS) codes, age group, and sex as features for the predictive model.



==> tex/clinical_scenario.tex <==
%  \todotip[PC]{lead}
Risk prediction models can be consumed by a broad spectrum of clinicians with differing roles and experience, e.g. a specialist vs a primary-care physician. Depending on their roles, the needs, and thereby the desired functionality from a risk prediction contextualization standpoint, can be different. As such, we conducted expert interview sessions
to understand the clinical use-case and determine the context of AI tools. More specifically,  we followed a sequence of %standard 
user-centric research principles~\cite{liao2020questioning}, to
(1) define the scope of our tool's capabilities, (2) identify the end-user/target persona who would most benefit from our tool, and (3) scope the most relevant %and realistic
contexts and usage scenarios for our tool.

Through our interviews, we identified primary-care physicians, especially those with lesser years of experience, to be the persona who may most benefit from such contextualizations. Based on these understandings, we formalize our use case to \textit{provide contextual explanations to a PCP around the predicted risk of {\ckd} among new {\dm} patients at their first diagnosis}.

==> tex/use_case.tex <==
% \todotip[PC]{lead}
% \explannote[PC]{done}
\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{images/ScientificAndContextualExample.png}
        \caption{Trace of dependencies of a contextual explanation example on system outputs from post-hoc explainer models and question-answering methods. In this example, we have used ontology classes and properties to annotate the data, but in this paper we mainly focus on a multi-method approach to support such contextual explanations.}
        \label{fig:usecaseexample}
\end{figure*}

Diabetes is one of the top five chronic diseases affecting the adult population in the US~\cite{cdcT2D}. 
Diabetes management involves monitoring for and treating %the 
related comorbid conditions. 
Effective and timely prediction of such conditions can lead to an overall improvement in the quality of care. We focus on {\dm} and use machine learning (ML) models to predict the risk of developing certain {\dm} comorbid complications. Among these, {\ckd}, a commonly occurring micro-vascular complication of {\dm}, is one of the leading causes of death in the US~\cite{cdcCKD}, with an estimated $37$ million cases in the US (who are mostly undiagnosed) and cost medicare in 2018 $81.1B$, and end stage renal disease an additional $36.6B$. Typically, actions to prevent onset of {\ckd} among {\dm} patients revolve around proper disease control,  including close disease monitoring, proper treatment adherence, and patient education. Incorporating accurate risk prediction of {\ckd} in the clinical workflow can lead to more timely actions, potentially delaying the onset of {\ckd}, and in some cases, preventing its progression.
While such predictions could be of use along various time-points of the patients' {\dm} prognosis, in this paper, we predict the risk of developing {\ckd} within 360 days of {\dm} onset. 
Under this use case, we explore strategies to provide context around interventions for particular patients, and explain their {\dm} state and individual risk factors.


